Runtime Monitoring of Dynamic Fairness Properties

A machine-learned system that is fair in static decision-making tasks may have biased societal impacts in the long-run. This may happen when the system interacts with humans and feedback patterns emerge, reinforcing old biases in the system and creating new biases. While existing works try to identify and mitigate long-run biases through smart system design, we introduce techniques for monitoring fairness in real time. Our goal is to build and deploy a monitor that will continuously observe a long sequence of events generated by the system in the wild, and will output, with each event, a verdict on how fair the system is at the current point in time. The advantages of monitoring are two-fold. Firstly, fairness is evaluated at run-time, which is important because unfair behaviors may not be eliminated a priori, at design-time, due to partial knowledge about the system and the environment, as well as uncertainties and dynamic changes in the system and the environment, such as the unpredictability of human behavior. Secondly, monitors are by design oblivious to how the monitored system is constructed, which makes them suitable to be used as trusted third-party fairness watchdogs. They function as computationally lightweight statistical estimators, and their correctness proofs rely on the rigorous analysis of the stochastic process that models the assumptions about the underlying dynamics of the system. We show, both in theory and experiments, how monitors can warn us (1) if a bank's credit policy over time has created an unfair distribution of credit scores among the population, and (2) if a resource allocator's allocation policy over time has made unfair allocations. Our experiments demonstrate that the monitors introduce very low overhead. We believe that runtime monitoring is an important and mathematically rigorous new addition to the fairness toolbox.

==> admission.tex <==
%!TEX root=main.tex

\section{A College Admission Problem}

Suppose there is a college that admits students based on their scores in an entrance examination.
At the beginning of each round of admission, the college announces the cutoff score for getting admission.
Every student has a true merit level, and for getting the admission, she can possibly improve her merit to achieve a score which is just sufficient for the admission, at the expense of a certain cost (for example, by investing in exam prep courses).
The cost that one needs to incur is proportional to the difference between her true merit and the cutoff level.
For every publicly known cutoff announced by the college, every student decides to either pay the cost or not with some probability.

The college wishes to admit only the truly meritorious students, and to safeguard against unmeritorious students from getting admissions through spending enough money.
To this end, the college may adopt robust policies that would increase the cutoff level.
Intuitively, this would result in a high cost that the unmeritorious students need to pay to adjust their scores, while making sure that it is still affordable for the truly meritorious ones.

Unfortunately, in some cases, such robust policies of the college were shown to treat unmeritorious students across different demographic groups unfairly.
We design a monitor that checks, in real-time, whether the college's policy has any adverse effect on the fairness, by observing the sequence of events comprising the college's cutoff, the observed scores of a sampled set of students, and the true merit levels of the same students as revealed in due course of time.

\subsection{Problem Formulation}

We formalize the problem in our framework as below:

\smallskip
\noindent\textbf{The agent and the environment:} 
In this example, the college plays the role of the agent, while the sampling of students and their manipulations of merit levels are controlled by the environment. 
Suppose the total number of students in a population sample at any given step is $N$ (the total number of applicants), the number of merit levels of the students is $K$, and there are two demographic groups $A$ and $B$ in the student population.
% merit thresholds for the students:
% the true one, denoted as , that is private to the college, and the robust one,
% denoted as $\pi\in [1\twodots K]$ with $\pi\geq \tau$, that is publicly announced and visible to the students.
% \KM{Is $\tau$ unknown to the monitor as well?}
We collect the distributions of true merits of students into two vectors based on their group identities. 
Namely, $\theta^A,\theta^B\in [0,1]^K$ are two vectors such that 
$\theta=\begin{bmatrix}
\theta^A\\
\theta^B
\end{bmatrix}$ 
is a simplex (i.e., $\sum_i \theta_i=1$), representing the distribution of true merits of students in the population.
%
%Suppose $\theta\in [0,1]^K\times \set{A,B}$ is a matrix whose element sum up to $1$ (i.e., $\sum_{k\in [1\twodots K]}\sum_{g\in \set{A,B}} \theta_{kg}=1$).
%The matrix $\theta$ representing the distribution of the true merit levels and the group identities among the population.
In other words, $\theta^g_{i}$, for $g\in \set{A,B}$, represents the probability that a student sampled uniformly at random from the population will have true merit $i$ and will belong to group $g$.
For any two merit levels $i,j$ with $j>i$, and for any group $g\in \set{A,B}$, let $p_{i}^g(j)$ and $c_i^g(j)$ denote the cost incurred by a student from group $g$ to go from the true merit level $i$ to the acquired merit level $j$, and the probability that she will actually pay this cost, respectively.


At every selection round, the following sequence of events take place:
\begin{enumerate}
	\item \textbf{Announcement of (public) merit threshold:} The college announces the public threshold $\tau_t$ greater or equal to the true threshold $\tau_*$.
	\item \textbf{Achieving threshold by incurring cost:} Let $S_t$ be a set of applicants sampled from the population of students.
	Given the public threshold, every student from $S_t$ in group $g$ with true merit $i<\tau_t$ acquires the merit $\tau_t$ by paying the cost $c_{i}^g(\tau_t)$ with probability $p_{i}^g(\tau_t)$.
%	Given the public threshold $\tau'$, the environment shifts the distribution of true merits $\theta$ to the distribution of acquired merits $\overline{\theta}$ as:
%\begin{align*}
%	\forall i \in [1\twodots K]\;.\;\forall g\in\set{A,B}\;.\;\overline{\theta}_{i}^{g} \coloneqq \begin{cases}
%															\theta_{i}^g(1-p^g_{i\tau'}) & i<\tau', \text{ i.e., students who choose not move to } \tau',\\
%															\theta_{i}^g +  \sum_{j < \tau'} \theta_{jg} p^g_{i\tau'} & i=\tau', \text{ i.e., students who move to from other levels } \tau',\\
%															\theta_{i}^g & i>\tau', \text{ i.e., students who do not need to move}.
%														\end{cases}
%\end{align*}
%It can be verified that $\overline{\theta}$ is a valid distribution, i.e., $\sum_i\overline{\theta}_{i} = 1$.
	\item \textbf{Selection and revelation of true merits:} The college selects the set of all students with acquired merit $\tau_t$, i.e.\ $S_t(\tau_t)$. After this the true merit of the accepted students is revealed. Each $X \in S_t(\tau_t)$ where every $X_i = \tup{k,g}$ is a tuple of the true merit $m\in [1\twodots K]$ and the group identity $g\in \set{A,B}$.
%	\item \textbf{Sampling applicants:} At every step, the environment generates a vector $X' \in \left([1\twodots K]\times \set{A,B}\right)^N$ based on samples drawn from the distribution $ \mathit{Categorical}(\overline{\theta})$: for every $i\in [1\twodots N]$, $\pr(X'_i=(x,g)) = \overline{\theta}_{x}^g$.
%Every element $X_i'$ of $X$ is the pair of the acquired skill level and the group identity of the $i$-th student in the sample.
%	\item \textbf{Selection process:} Let $Y' = \set{Y_1',\ldots,Y_m'}$ be the subset of the selected sample $X'$ such that for every $i\in [1\twodots m]$, if $Y_i'=(y,g)$ then $y\geq \tau'$, i.e., $Y'$ denotes the set of students from both groups who were admitted to the college.
%Suppose $\set{y_1',\ldots,y_m'}$ is the set of  acquired merits of the respective admitted students $\set{Y_1',\ldots,Y_m'}$.
%	\item \textbf{Revelation of true merits:} Subsequently, the true merits of the students get revealed (through the college's curriculum), which are denoted as $\set{y_1,\ldots,y_m}$.
\end{enumerate}
\KK{I think you ment conditional probability. I changed it here but it has to be changed above as well.}
\KK{We need to change that. I dont know how exactly}
\smallskip
\noindent\textbf{The fairness property:}
Define social burden of a group $g\in \set{A,B}$ as the expected cost that every truly meritorious student (i.e., a student with true merit greater than $\tau^*$) needs to incur in order to get admitted in the college, formalized as
 $\expe(c_{i}^g(\tau_t)\mid i\geq \tau) = \sum_{i= \tau_t}^K c_{i}^g(\tau_t)\cdot \pr(i\mid g)$, where $\pr(i\mid g)$ is the probability that a student sampled from the population has true merit $i$ and belongs to group $g$, and is equal to the (unknown) conditional distribution parameter $\theta_i^g$.
Since $\pr(i,g) =0$ for $i\geq \tau'$, hence we can equivalently compute the sum up to $\tau'-1$ and write $\expe(c_{i\tau'-1}^g\mid i\geq \tau) = \sum_{i= \tau}^{\tau'-1} c_{i\tau'}^g\cdot \pr(i,g)$.
\KM{I cannot get rid of the $\tau$ from the definition, which means that $\tau$ needs to be known to the monitor somehow.}
The fairness property that we consider is the disparity in the social burden across the two groups $A$ and $B$, formalized using the following expression:
\begin{align*}
	\varphi \coloneqq \expe(c_{i\tau'}^A\mid i\geq \tau) - \expe(c_{i\tau'}^B\mid i\geq \tau).
\end{align*}
\KM{Here $\tau'$ is changing over time, which means that $\varphi$ is a function over $\tau'$. How to use that in the specification? Is it ``$\forall \tau'$"?}

\subsection{The Runtime Monitor}

We construct a runtime monitor that estimates the value of $\varphi$ at runtime.
The parameters that used for constructing the monitor are: 
$\tau$, 
$p_{i}^g(j)$, $c_{i}^g(j)$, for $g\in \set{A,B}$ and for every $i,j\in [1\twodots K]$,
and a parameter $\delta\in [0,1]$.
At runtime, at every step, the monitor receives the following inputs:
(i) the new announced threshold $\tau_t$ and
(ii) the new set of admitted students $S_t(\tau_t)$.
The output of the monitor is a confidence interval estimate for $\varphi$ with a given confidence level $1-\delta$.
The more number of admission cycles the monitor watches, the tighter the confidence interval gets.

First, fix a group $g\in \set{A,B}$, and we show how to estimate the social burden of group $g$.
The aim of the monitor is to compute the conditional expectation 


%We assume that $\tau$, $\tau'$, $p_{i\tau'}^g$, $c_{i\tau'}^g$, for $g\in \set{A,B}$, are known to the monitor.
Observe that the social burden can be written as $\expe(c_{i\tau'}^g\mid i\geq \tau) = \sum_{i=\tau}^{\tau'-1} c_{i\tau'}^g\cdot \pr(i,g) = \sum_{i= \tau}^{\tau'-1} c_{i\tau'}^g\cdot \theta_{i}^g$.
%If we were able to directly estimate $\theta_{ig}$, then we could use these estimates to compute the social burden of each group.
%However, the monitor only sees samples from the altered distribution $\mathit{Categorical}(\theta')$, and thus can only estimate $\theta'$. 
Thus, if we can estimate $\theta_{i}^g$ (the distribution of true merits), we will be able to estimate the social burden of group $g$.

We pick a student uniformly at random from the set of admitted students, and let the probability that the chosen student belongs to the group $g$ and has a true merit $i$ be denoted as $q_{i}^g$.
If $i<\tau'$, then we know that the chosen student is among those who incurred the cost that was needed to achieve the threshold level $\tau'$.
Thus, we have $q_i^g = \theta_i^g\cdot p_i^g$, from which we obtain $\theta_i^g = \sfrac{q_i^g}{p_i^g}$.
Moreover, $q_i^g$ can be empirically estimated within a confidence interval with any arbitrary confidence level, by computing the average number of admitted students from group $g$ and with true merit $i$ from the sequence of sets of admitted students $\set{X_1^1,\ldots,X_m^1},\ldots,\set{X_1^l,\ldots,X_m^l}$, and through the application of Hoeffding's inequality. 
This gives us an interval estimate for $q_i^g$ for every $i$, which in turn can be used to estimate $\theta_i^g$, followed by the social burden on group $g$, followed by the disparity in social burden between the two groups.

The monitoring algorithm is summarized in Alg.~\ref{?}.




\begin{algorithm}
		\caption{The monitor for the college admission example}
	\label{alg:lending monitor}
	\begin{minipage}{0.45\textwidth}
		\begin{algorithmic}[1]
			\Function{$\mathtt{Init\_memory}()$}{}
				\State $t\gets 0$ \Comment{clock counters}
				\State $\set{\hat{q}_i^g\gets 0}_{i\in [1\twodots K],\, g\in\set{A,B}}$ \Comment{emp.\ est.\ of $q_i^g$-s}
%				\State $\overline{\mu}_A,\overline{\mu}_B\gets 0$ \Comment{emp.\ av.\ true merits}
			\EndFunction
		\end{algorithmic}
	\end{minipage}
	\begin{minipage}{0.45\textwidth}
		\begin{algorithmic}[1]
			\Function{$\mathtt{Compute}_\delta$}{$\set{(k_1,g_1),\ldots,(k_m,g_m)},\Delta$}
				\State $t\gets t+1$
				\For{$g\in \set{A,B}$}
					\For{$k\in [1\twodots K]$}
						\State $c \gets \frac{1}{m}\sum_{i=1}^m \mathbbm{1}(k_i=k,g_i=g)$
						\State $\hat{q}_k^g\gets \frac{1}{t}\left(q_k^g(t-1) + c\right)$
						\State $\hat{\theta}_k^g \gets \frac{\hat{q}_k^g}{p_{k}^g}$
					\EndFor
				\EndFor	
				\State $\hat{E}^A\gets \sum_{k=\tau}^{\tau'-1} c_{k\tau'}^A\cdot \hat{\theta}_k^A$
				\State $\hat{E}^B\gets \sum_{k=\tau}^{\tau'-1} c_{k\tau'}^B\cdot \hat{\theta}_k^B$
				\State $\hat{E} \gets \hat{E}^A-\hat{E}^B$
				\State \todo{the error?}
				\State \Return \todo{}			
			\EndFunction
		\end{algorithmic}
	\end{minipage}
\end{algorithm}


\section{New algorithm}

\begin{algorithm}
	\caption{The monitor for the college admission example}
\label{alg:lending monitor}
\begin{minipage}{0.45\textwidth}
	\begin{algorithmic}[1]
		\Function{$\mathtt{Init\_memory}()$}{}
			\State $t\gets 0$ \Comment{clock counters}
			\State $\set{\hat{q}_i^g\gets 0}_{i\in [1\twodots K],\, g\in\set{A,B}}$ \Comment{emp.\ est.\ of $q_i^g$-s}
%				\State $\overline{\mu}_A,\overline{\mu}_B\gets 0$ \Comment{emp.\ av.\ true merits}
		\EndFunction
	\end{algorithmic}
\end{minipage}
\begin{minipage}{0.45\textwidth}
	\begin{algorithmic}[1]
		\Function{$\mathtt{Compute}_\delta$}{$\set{(k_1,g_1),\ldots,(k_m,g_m)},\Delta$}
			\State $t\gets t+1$
			\For{$g\in \set{A,B}$}
				\For{$k\in [1\twodots K]$}
					\State $c \gets \frac{1}{m}\sum_{i=1}^m \mathbbm{1}(k_i=k,g_i=g)$
					\State $\hat{q}_k^g\gets \frac{1}{t}\left(q_k^g(t-1) + c\right)$
					\State $\hat{\theta}_k^g \gets \frac{\hat{q}_k^g}{p_{k}^g}$
				\EndFor
			\EndFor	
			\State $\hat{E}^A\gets \sum_{k=\tau}^{\tau'-1} c_{k\tau'}^A\cdot \hat{\theta}_k^A$
			\State $\hat{E}^B\gets \sum_{k=\tau}^{\tau'-1} c_{k\tau'}^B\cdot \hat{\theta}_k^B$
			\State $\hat{E} \gets \hat{E}^A-\hat{E}^B$
			\State \todo{the error?}
			\State \Return \todo{}			
		\EndFunction
	\end{algorithmic}
\end{minipage}
\end{algorithm}


%It would be a straightforward task to estimate $\theta_{ig}$, if the monitor were able to observe samples from the distribution $\mathit{Categorical}(\theta_{ig})$.
%Instead, the monitor observes samples $X'$ from the modified distribution $\mathit{Categorical}(\theta_{ig}')$.
%In the end, the monitor gets to see the true merit levels $\set{y_1,\ldots,y_m}$ for a subset $Y'$ of students in $X'$.
%Let $A^g\coloneqq \sfrac{1}{m}\cdot \sum_{i=1}^m \mathbbm{1}(y_i=x,Y_i'=g)$ be an empirical estimator for the average number of students from $g$ with true merit $x$ getting admitted to the college.
%Since, we know that $p_{i\tau'}^g$ fraction of the  students from group $g$ and true merit $x$ increased their acquired merits and got admitted, we obtain $p_{i\tau'}^g\cdot \theta_{ig} = A^g$, which gives us an empirical estimator of $\theta_{ig}$ as $\hat{\theta}_{ig} = \sfrac{A^g}{p_{i\tau'}^g}$.

\subsection{Experimental Outcome}



\subsection{The Runtime Monitor}

\begin{algorithm}
		\caption{The monitor for the college admission example}
	\label{alg:lending monitor}
	\begin{minipage}{0.45\textwidth}
		\begin{algorithmic}[1]
			\Function{$\mathtt{Init\_memory}()$}{}
				\State $t\gets 0$ \Comment{clock counters}
				\State $\set{\hat{q}_i^g\gets 0}_{i\in [1\twodots K],\, g\in\set{A,B}}$ \Comment{emp.\ est.\ of $q_i^g$-s}
%				\State $\overline{\mu}_A,\overline{\mu}_B\gets 0$ \Comment{emp.\ av.\ true merits}
			\EndFunction
		\end{algorithmic}
	\end{minipage}
	\begin{minipage}{0.45\textwidth}
		\begin{algorithmic}[1]
			\Function{$\mathtt{Compute}_\delta$}{$\set{(k_1,g_1),\ldots,(k_m,g_m)},\Delta$}
				\State $t\gets t+1$
				\For{$g\in \set{A,B}$}
					\For{$k\in [1\twodots K]$}
						\State $c \gets \frac{1}{m}\sum_{i=1}^m \mathbbm{1}(k_i=k,g_i=g)$
						\State $\hat{q}_k^g\gets \frac{1}{t}\left(q_k^g(t-1) + c\right)$
						\State $\hat{\theta}_k^g \gets \frac{\hat{q}_k^g}{p_{k}^g}$
					\EndFor
				\EndFor	
				\State $\hat{E}^A\gets \sum_{k=\tau}^{\tau'-1} c_{k\tau'}^A\cdot \hat{\theta}_k^A$
				\State $\hat{E}^B\gets \sum_{k=\tau}^{\tau'-1} c_{k\tau'}^B\cdot \hat{\theta}_k^B$
				\State $\hat{E} \gets \hat{E}^A-\hat{E}^B$
				\State \todo{the error?}
				\State \Return \todo{}			
			\EndFunction
		\end{algorithmic}
	\end{minipage}
\end{algorithm}



% %!TEX root=main.tex

% \section{A College Admission Problem}

% Suppose there is a college that admits students based on their scores in an entrance examination.
% At the beginning of each round of admission, the college announces the cutoff score for getting admission.
% Every student has a true merit level, and for getting the admission, she can possibly improve her merit to achieve a score which is just sufficient for the admission, at the expense of a certain cost (for example, by investing in exam prep courses).
% The cost that one needs to incur is proportional to the difference between her true merit and the cutoff level.
% For every publicly known cutoff announced by the college, every student decides to either pay the cost or not with some probability.

% The college wishes to admit only the truly meritorious students, and to safeguard against unmeritorious students from getting admissions through spending enough money.
% To this end, the college may adopt robust policies that would increase the cutoff level.
% Intuitively, this would result in a high cost that the unmeritorious students need to pay to adjust their scores, while making sure that it is still affordable for the truly meritorious ones.

% Unfortunately, in some cases, such robust policies of the college were shown to treat unmeritorious students across different demographic groups unfairly.
% We design a monitor that checks, in real-time, whether the college's policy has any adverse effect on the fairness, by observing the sequence of events comprising the college's cutoff, the observed scores of a sampled set of students, and the true merit levels of the same students as revealed in due course of time.

% \subsection{Problem Formulation}

% We formalize the problem in our framework as below:

% \smallskip
% \noindent\textbf{The agent and the environment:} 
% In this example, the college plays the role of the agent, while the sampling of students and their manipulations of merit levels are controlled by the environment. 
% Suppose the total number of students in a population sample at any given step is $N$ (the total number of applicants), the number of merit levels of the students is $K$, and there are two demographic groups $A$ and $B$ in the student population.
% % merit thresholds for the students:
% % the true one, denoted as , that is private to the college, and the robust one,
% % denoted as $\pi\in [1\twodots K]$ with $\pi\geq \tau$, that is publicly announced and visible to the students.
% % \KM{Is $\tau$ unknown to the monitor as well?}
% We collect the distributions of true merits of students into two vectors based on their group identities. 
% Namely, $\theta^A,\theta^B\in [0,1]^K$ are two vectors such that 
% $\theta=\begin{bmatrix}
% \theta^A\\
% \theta^B
% \end{bmatrix}$ 
% is a simplex (i.e., $\sum_i \theta_i=1$), representing the distribution of true merits of students in the population.
% %
% %Suppose $\theta\in [0,1]^K\times \set{A,B}$ is a matrix whose element sum up to $1$ (i.e., $\sum_{k\in [1\twodots K]}\sum_{g\in \set{A,B}} \theta_{kg}=1$).
% %The matrix $\theta$ representing the distribution of the true merit levels and the group identities among the population.
% In other words, $\theta^g_{i}$, for $g\in \set{A,B}$, represents the probability that a student sampled uniformly at random from the population will have true merit $i$ and will belong to group $g$.
% For any two merit levels $i,j$ with $j>i$, and for any group $g\in \set{A,B}$, let $p_{i}^g(j)$ and $c_i^g(j)$ denote the cost incurred by a student from group $g$ to go from the true merit level $i$ to the acquired merit level $j$, and the probability that she will actually pay this cost, respectively.


% At every selection round, the following sequence of events take place:
% \begin{enumerate}
% 	\item \textbf{Announcement of (public) merit threshold:} The college announces the public threshold $\tau_t$ greater or equal to the true threshold $\tau_*$.
% 	\item \textbf{Achieving threshold by incurring cost:} Let $S_t$ be a set of applicants sampled from the population of students.
% 	Given the public threshold, every student from $S_t$ in group $g$ with true merit $i<\tau_t$ acquires the merit $\tau_t$ by paying the cost $c_{i}^g(\tau_t)$ with probability $p_{i}^g(\tau_t)$.
% %	Given the public threshold $\tau'$, the environment shifts the distribution of true merits $\theta$ to the distribution of acquired merits $\overline{\theta}$ as:
% %\begin{align*}
% %	\forall i \in [1\twodots K]\;.\;\forall g\in\set{A,B}\;.\;\overline{\theta}_{i}^{g} \coloneqq \begin{cases}
% %															\theta_{i}^g(1-p^g_{i\tau'}) & i<\tau', \text{ i.e., students who choose not move to } \tau',\\
% %															\theta_{i}^g +  \sum_{j < \tau'} \theta_{jg} p^g_{i\tau'} & i=\tau', \text{ i.e., students who move to from other levels } \tau',\\
% %															\theta_{i}^g & i>\tau', \text{ i.e., students who do not need to move}.
% %														\end{cases}
% %\end{align*}
% %It can be verified that $\overline{\theta}$ is a valid distribution, i.e., $\sum_i\overline{\theta}_{i} = 1$.
% 	\item \textbf{Selection and revelation of true merits:} The college selects the set of all students with acquired merit $\tau_t$, i.e.\ $S_t(\tau_t)$. After this the true merit of the accepted students is revealed. Each $X \in S_t(\tau_t)$ where every $X_i = \tup{k,g}$ is a tuple of the true merit $m\in [1\twodots K]$ and the group identity $g\in \set{A,B}$.
% %	\item \textbf{Sampling applicants:} At every step, the environment generates a vector $X' \in \left([1\twodots K]\times \set{A,B}\right)^N$ based on samples drawn from the distribution $ \mathit{Categorical}(\overline{\theta})$: for every $i\in [1\twodots N]$, $\pr(X'_i=(x,g)) = \overline{\theta}_{x}^g$.
% %Every element $X_i'$ of $X$ is the pair of the acquired skill level and the group identity of the $i$-th student in the sample.
% %	\item \textbf{Selection process:} Let $Y' = \set{Y_1',\ldots,Y_m'}$ be the subset of the selected sample $X'$ such that for every $i\in [1\twodots m]$, if $Y_i'=(y,g)$ then $y\geq \tau'$, i.e., $Y'$ denotes the set of students from both groups who were admitted to the college.
% %Suppose $\set{y_1',\ldots,y_m'}$ is the set of  acquired merits of the respective admitted students $\set{Y_1',\ldots,Y_m'}$.
% %	\item \textbf{Revelation of true merits:} Subsequently, the true merits of the students get revealed (through the college's curriculum), which are denoted as $\set{y_1,\ldots,y_m}$.
% \end{enumerate}
% \KK{I think you ment conditional probability. I changed it here but it has to be changed above as well.}
% \KK{We need to change that. I dont know how exactly}
% \smallskip
% \noindent\textbf{The fairness property:}
% Define social burden of a group $g\in \set{A,B}$ as the expected cost that every truly meritorious student (i.e., a student with true merit greater than $\tau^*$) needs to incur in order to get admitted in the college, formalized as
%  $\expe(c_{i}^g(\tau_t)\mid i\geq \tau) = \sum_{i= \tau_t}^K c_{i}^g(\tau_t)\cdot \pr(i\mid g)$, where $\pr(i\mid g)$ is the probability that a student sampled from the population has true merit $i$ and belongs to group $g$, and is equal to the (unknown) conditional distribution parameter $\theta_i^g$.
% Since $\pr(i,g) =0$ for $i\geq \tau'$, hence we can equivalently compute the sum up to $\tau'-1$ and write $\expe(c_{i\tau'-1}^g\mid i\geq \tau) = \sum_{i= \tau}^{\tau'-1} c_{i\tau'}^g\cdot \pr(i,g)$.
% \KM{I cannot get rid of the $\tau$ from the definition, which means that $\tau$ needs to be known to the monitor somehow.}
% The fairness property that we consider is the disparity in the social burden across the two groups $A$ and $B$, formalized using the following expression:
% \begin{align*}
% 	\varphi \coloneqq \expe(c_{i\tau'}^A\mid i\geq \tau) - \expe(c_{i\tau'}^B\mid i\geq \tau).
% \end{align*}
% \KM{Here $\tau'$ is changing over time, which means that $\varphi$ is a function over $\tau'$. How to use that in the specification? Is it ``$\forall \tau'$"?}

% \subsection{The Runtime Monitor}

% We construct a runtime monitor that estimates the value of $\varphi$ at runtime.
% The parameters that used for constructing the monitor are: 
% $\tau$, 
% $p_{i}^g(j)$, $c_{i}^g(j)$, for $g\in \set{A,B}$ and for every $i,j\in [1\twodots K]$,
% and a parameter $\delta\in [0,1]$.
% At runtime, at every step, the monitor receives the following inputs:
% (i) the new announced threshold $\tau_t$ and
% (ii) the new set of admitted students $S_t(\tau_t)$.
% The output of the monitor is a confidence interval estimate for $\varphi$ with a given confidence level $1-\delta$.
% The more number of admission cycles the monitor watches, the tighter the confidence interval gets.

% First, fix a group $g\in \set{A,B}$, and we show how to estimate the social burden of group $g$.
% The aim of the monitor is to compute the conditional expectation 
% \begin{align*}
	
% \end{align*}

% %We assume that $\tau$, $\tau'$, $p_{i\tau'}^g$, $c_{i\tau'}^g$, for $g\in \set{A,B}$, are known to the monitor.
% Observe that the social burden can be written as $\expe(c_{i\tau'}^g\mid i\geq \tau) = \sum_{i=\tau}^{\tau'-1} c_{i\tau'}^g\cdot \pr(i,g) = \sum_{i= \tau}^{\tau'-1} c_{i\tau'}^g\cdot \theta_{i}^g$.
% %If we were able to directly estimate $\theta_{ig}$, then we could use these estimates to compute the social burden of each group.
% %However, the monitor only sees samples from the altered distribution $\mathit{Categorical}(\theta')$, and thus can only estimate $\theta'$. 
% Thus, if we can estimate $\theta_{i}^g$ (the distribution of true merits), we will be able to estimate the social burden of group $g$.

% We pick a student uniformly at random from the set of admitted students, and let the probability that the chosen student belongs to the group $g$ and has a true merit $i$ be denoted as $q_{i}^g$.
% If $i<\tau'$, then we know that the chosen student is among those who incurred the cost that was needed to achieve the threshold level $\tau'$.
% Thus, we have $q_i^g = \theta_i^g\cdot p_i^g$, from which we obtain $\theta_i^g = \sfrac{q_i^g}{p_i^g}$.
% Moreover, $q_i^g$ can be empirically estimated within a confidence interval with any arbitrary confidence level, by computing the average number of admitted students from group $g$ and with true merit $i$ from the sequence of sets of admitted students $\set{X_1^1,\ldots,X_m^1},\ldots,\set{X_1^l,\ldots,X_m^l}$, and through the application of Hoeffding's inequality. 
% This gives us an interval estimate for $q_i^g$ for every $i$, which in turn can be used to estimate $\theta_i^g$, followed by the social burden on group $g$, followed by the disparity in social burden between the two groups.

% The monitoring algorithm is summarized in Alg.~\ref{?}.

% \begin{algorithm}
% 		\caption{The monitor for the college admission example}
% 	\label{alg:lending monitor}
% 	\begin{minipage}{0.45\textwidth}
% 		\begin{algorithmic}[1]
% 			\Function{$\mathtt{Init\_memory}()$}{}
% 				\State $t\gets 0$ \Comment{clock counters}
% 				\State $\set{\hat{q}_i^g\gets 0}_{i\in [1\twodots K],\, g\in\set{A,B}}$ \Comment{emp.\ est.\ of $q_i^g$-s}
% %				\State $\overline{\mu}_A,\overline{\mu}_B\gets 0$ \Comment{emp.\ av.\ true merits}
% 			\EndFunction
% 		\end{algorithmic}
% 	\end{minipage}
% 	\begin{minipage}{0.45\textwidth}
% 		\begin{algorithmic}[1]
% 			\Function{$\mathtt{Compute}_\delta$}{$\set{(k_1,g_1),\ldots,(k_m,g_m)},\Delta$}
% 				\State $t\gets t+1$
% 				\For{$g\in \set{A,B}$}
% 					\For{$k\in [1\twodots K]$}
% 						\State $c \gets \frac{1}{m}\sum_{i=1}^m \mathbbm{1}(k_i=k,g_i=g)$
% 						\State $\hat{q}_k^g\gets \frac{1}{t}\left(q_k^g(t-1) + c\right)$
% 						\State $\hat{\theta}_k^g \gets \frac{\hat{q}_k^g}{p_{k}^g}$
% 					\EndFor
% 				\EndFor	
% 				\State $\hat{E}^A\gets \sum_{k=\tau}^{\tau'-1} c_{k\tau'}^A\cdot \hat{\theta}_k^A$
% 				\State $\hat{E}^B\gets \sum_{k=\tau}^{\tau'-1} c_{k\tau'}^B\cdot \hat{\theta}_k^B$
% 				\State $\hat{E} \gets \hat{E}^A-\hat{E}^B$
% 				\State \todo{the error?}
% 				\State \Return \todo{}			
% 			\EndFunction
% 		\end{algorithmic}
% 	\end{minipage}
% \end{algorithm}

% %It would be a straightforward task to estimate $\theta_{ig}$, if the monitor were able to observe samples from the distribution $\mathit{Categorical}(\theta_{ig})$.
% %Instead, the monitor observes samples $X'$ from the modified distribution $\mathit{Categorical}(\theta_{ig}')$.
% %In the end, the monitor gets to see the true merit levels $\set{y_1,\ldots,y_m}$ for a subset $Y'$ of students in $X'$.
% %Let $A^g\coloneqq \sfrac{1}{m}\cdot \sum_{i=1}^m \mathbbm{1}(y_i=x,Y_i'=g)$ be an empirical estimator for the average number of students from $g$ with true merit $x$ getting admitted to the college.
% %Since, we know that $p_{i\tau'}^g$ fraction of the  students from group $g$ and true merit $x$ increased their acquired merits and got admitted, we obtain $p_{i\tau'}^g\cdot \theta_{ig} = A^g$, which gives us an empirical estimator of $\theta_{ig}$ as $\hat{\theta}_{ig} = \sfrac{A^g}{p_{i\tau'}^g}$.

% \subsection{Experimental Outcome}



% \subsection{The Runtime Monitor}

% \begin{algorithm}
% 		\caption{The monitor for the college admission example}
% 	\label{alg:lending monitor}
% 	\begin{minipage}{0.45\textwidth}
% 		\begin{algorithmic}[1]
% 			\Function{$\mathtt{Init\_memory}()$}{}
% 				\State $t\gets 0$ \Comment{clock counters}
% 				\State $\set{\hat{q}_i^g\gets 0}_{i\in [1\twodots K],\, g\in\set{A,B}}$ \Comment{emp.\ est.\ of $q_i^g$-s}
% %				\State $\overline{\mu}_A,\overline{\mu}_B\gets 0$ \Comment{emp.\ av.\ true merits}
% 			\EndFunction
% 		\end{algorithmic}
% 	\end{minipage}
% 	\begin{minipage}{0.45\textwidth}
% 		\begin{algorithmic}[1]
% 			\Function{$\mathtt{Compute}_\delta$}{$\set{(k_1,g_1),\ldots,(k_m,g_m)},\Delta$}
% 				\State $t\gets t+1$
% 				\For{$g\in \set{A,B}$}
% 					\For{$k\in [1\twodots K]$}
% 						\State $c \gets \frac{1}{m}\sum_{i=1}^m \mathbbm{1}(k_i=k,g_i=g)$
% 						\State $\hat{q}_k^g\gets \frac{1}{t}\left(q_k^g(t-1) + c\right)$
% 						\State $\hat{\theta}_k^g \gets \frac{\hat{q}_k^g}{p_{k}^g}$
% 					\EndFor
% 				\EndFor	
% 				\State $\hat{E}^A\gets \sum_{k=\tau}^{\tau'-1} c_{k\tau'}^A\cdot \hat{\theta}_k^A$
% 				\State $\hat{E}^B\gets \sum_{k=\tau}^{\tau'-1} c_{k\tau'}^B\cdot \hat{\theta}_k^B$
% 				\State $\hat{E} \gets \hat{E}^A-\hat{E}^B$
% 				\State \todo{the error?}
% 				\State \Return \todo{}			
% 			\EndFunction
% 		\end{algorithmic}
% 	\end{minipage}
% \end{algorithm}


==> general.tex <==
% !TEX root=main.tex

\section{General Algorithm}
In this section we present a monitoring algorithm for a general class of stochastic processes which is defined as follows.
Let $Z \coloneqq (Z_t)_{t\in [T]}$ be a sequence random variables over $\Omega$ where $[T]=[1,2,\dots,T]$ for some $T\in \mathbb{N}$. We require from $\Omega$ that for any $t\in [T]$ we have $Z_t=(X_t,Y_t)$ where both random variables are discrete and $X_t$ has support $\mathbb{N}$ and bounded expectation.
Moreover, we require the that there exists a function $\tau: \Omega \to \mathbb{R}$ such that for any $t\in [T-1]$ and any sequence $z=(z_1,\dots,z_{t})\in \Omega^{t}$ 
\begin{align*}
\expe\left( X_{t+1} \middle| \{Z=z\}_t\right) = \expe\left( X_{t} \middle| Z_1=z_1, \dots,Z_{t-1}=z_{t-1}\right) + \tau(z_t)
\end{align*}


For this class of processes we are able to estimate $\expe\left( X_1 \right)$ using an estimator that accounts for the observed changes in expectation, i.e.\
\begin{align*}
	\hat{E} \coloneqq \frac{1}{T} \sum_{t=1}^{T} X_t - \sum_{i=1}^{t-1} \tau(Z_i)
\end{align*}
The error of this estimator can be bounded using Doob-martingales and 
a variant of Azumas inequality suitable for a sub-exponentially distributed martingale difference sequences. 
% We show that under the assumption that $X_t$ is a sub-exponential random variable our monitor provides formally correct results. 
As a consequence, our monitor is suitable for cases where $X_t$ is a bounded, sub-gaussian or sub-exponential random variable. Thereby covering a wide range of commonly used distributions.

From a monitoring perspective, estimating $\expe(E_1)$ is not particularly interesting. However, using the estimate of $\expe(X_1)$ and the sequence $\tau(z_1), \dots, \tau(z_{T-1})$, we are able to estimate $\expe\left(X_T \middle|  Z_1=z_1, \dots,Z_{T-1}=z_{T-1}\right)$ with the same error, by adding the concrete sequence of differences to $\hat{E}$. 


In its most general form, we consider $K \in \mathbb{N}$ independent stochastic processes. Let $\hat{E}_1, \dots, \hat{E}_K$ be the estimators of the respective processes. Our monitor is designed to handel arbitrary linear combinations over those estimators. 



\begin{algorithm}
	\caption{\texttt{Monitor}}
	\label{alg:monitor_general}
	\begin{minipage}{0.45\textwidth}
		\begin{algorithmic}[1]
			\Require $\delta, \tau$
			\Function{$\mathtt{Init}$}{}
				% \State $\delta \gets \delta$ \Comment{the target confidence level}
				% \State $\{\gamma_k\gets \gamma_k\}_{k\in[K]}$ \Comment{constants in the sum}
				\State $\{T_k\gets 0\}_{k\in[K]}$ \Comment{clock counters}
				\State $\{\hat{E}_k\gets 0\}_{k\in[K]}$ \Comment{Estimators at time $0$.}
				\State $\{d_k\gets 0\}_{k\in[K]}$ \Comment{net distribution shifts}
				% \State $\{\sigma^2_k\gets \sigma^2_k\}_{k\in[K]}$
				% \State $\{\nu_k\gets \nu_k\}_{k\in[K]}$
%				\State $\varepsilon\gets \bot$ \Comment{est.\ error, init.\ w/ dummy symbol}
			\EndFunction
		\end{algorithmic}
	\end{minipage}
	\begin{minipage}{0.45\textwidth}
		\begin{algorithmic}[1]
			\Function{$\mathtt{Compute}$}{$k,(x,y)$}
			\State $T_k\gets T_k+1$
			\If{$\min_k(T_k)=0$} 
			\State \Return $?$
			\EndIf
			\State $\hat{E}_k\gets \frac{1}{T_k}\left(\hat{E}_k \cdot (T_k-1)+ (x-d_k)\right)$ \label{alg:line:moving av. a}
			\Comment{moving average computation of $\hat{E}_k$}
			\State $\hat{\varphi} \gets  \sum_{k=1}^{K} \gamma_k \cdot (\hat{E}_k + d_k) $  \Comment{emp.\ estimate of $\varphi$} 
			\State $d_k\gets d_k + \tau((x,y))$ \Comment{expectation shift}
			\State $\varepsilon_{\sigma^2} \gets \sqrt{2\cdot \sum_{k=1}^K \gamma_k^2\cdot\frac{\sigma_k^2}{T_k} \cdot \ln\left( \frac{2}{\delta}\right)} $
			\State $\varepsilon_{\nu} \gets 2\cdot \max_k\left(\frac{\nu_k}{T_k}\right) \cdot \ln\left( \frac{2}{\delta}\right)$
			\State $\varepsilon \gets \max(\varepsilon_{\sigma^2}, \varepsilon_{\nu})$ \Comment{Computation of error}
				\State \Return $[\overline{\varphi}-\varepsilon,\overline{\varphi}+\varepsilon]$ \Comment{return the conf.\ int.}
			\EndFunction
		\end{algorithmic}
	\end{minipage}
\end{algorithm}




\begin{algorithm}
	\caption{\texttt{Monitor}}
	\label{alg:monitor_general}
	\begin{minipage}{0.45\textwidth}
		\begin{algorithmic}[1]
			\Require \\
			$(\gamma_k)_{k\in [K]}$ \Comment{constants of the wieghted sum} \\
			$\delta$, \Comment{confidence} \\
			$(\tau_k)_{k\in [K]}$, \Comment{functions to compute the shift in expectation} \\
			 $(\sigma_k^2,\nu_k)_{k\in [K]}$,  \Comment{sub-exponential parameter}\\
			\Function{$\mathtt{Init}$}{}
				% \State $\delta \gets \delta$ \Comment{the target confidence level}
				% \State $\{\gamma_k\gets \gamma_k\}_{k\in[K]}$ \Comment{constants in the sum}
				\State $\{T_k\gets 0\}_{k\in[K]}$ \Comment{clock counters}
				\State $\{\hat{E}_k\gets 0\}_{k\in[K]}$ \Comment{Estimators at time $0$.}
				\State $\{d_k\gets 0\}_{k\in[K]}$ \Comment{net distribution shifts}
				% \State $\{\sigma^2_k\gets \sigma^2_k\}_{k\in[K]}$
				% \State $\{\nu_k\gets \nu_k\}_{k\in[K]}$
%				\State $\varepsilon\gets \bot$ \Comment{est.\ error, init.\ w/ dummy symbol}
			\EndFunction
		\end{algorithmic}
	\end{minipage}
	\begin{minipage}{0.45\textwidth}
		\begin{algorithmic}[1]
			\Function{$\mathtt{Compute}$}{$k,(x,y)$}
			\State $T_k\gets T_k+1$
			\If{$\min_k(T_k)=0$} 
			\State \Return $?$
			\EndIf
			\State $\hat{E}_k\gets \frac{1}{T_k}\left(\hat{E}_k \cdot (T_k-1)+ (x-d_k)\right)$ \label{alg:line:moving av. a}
			\Comment{moving average computation of $\hat{E}_k$}
			\State $\hat{\varphi} \gets  \sum_{k=1}^{K} \gamma_k \cdot (\hat{E}_k + d_k) $  \Comment{emp.\ estimate of $\varphi$} 
			\State $d_k\gets d_k + \tau((x,y))$ \Comment{expectation shift}
			\State $\varepsilon_{\sigma^2} \gets \sqrt{2\cdot \sum_{k=1}^K \gamma_k^2\cdot\frac{\sigma_k^2}{T_k} \cdot \ln\left( \frac{2}{\delta}\right)} $
			\State $\varepsilon_{\nu} \gets 2\cdot \max_k\left(\frac{\nu_k}{T_k}\right) \cdot \ln\left( \frac{2}{\delta}\right)$
			\State $\varepsilon \gets \max(\varepsilon_{\sigma^2}, \varepsilon_{\nu})$ \Comment{Computation of error}
				\State \Return $[\overline{\varphi}-\varepsilon,\overline{\varphi}+\varepsilon]$ \Comment{return the conf.\ int.}
			\EndFunction
		\end{algorithmic}
	\end{minipage}
\end{algorithm}



==> prelims.tex <==
%!TEX root=main.tex
\section{Preliminaries}
We write $\mathbb{R}$, $\mathbb{R}^+$, $\mathbb{N}$, and $\mathbb{N}^+$ to denote the sets of real numbers, positive real numbers, natural numbers (including zero), and positive integers respectively.

Suppose $S_X = (\Omega_X,\mathcal{F}_X,\pr_X)$ and $S_Y=(\Omega_Y,\mathcal{F}_Y,\pr_Y)$ are a pair of probability spaces. Let $Y\colon \Omega_Y\to \mathbb{R}$ be a random variable defined on $S_Y$, and $Z\colon \Omega_X\times \Omega_Y\to \mathbb{R}$ be a random variable on the product probability space of $S_X$ and $S_Y$.
We use $(Z\mid Y=y)$, for $y\in \Omega_Y$, to denote the random variable over $S_X$ which is obtained by restricting $Z$ to $Y=y$ in its $Y$-component; formally, for $\omega\in\Omega_X$, $(Z\mid Y=y)(\omega) = Z(\omega,y)$.


==> theory.tex <==
% !TEX root=main.tex

%\section{The Approach}
%
%%We solve Prob.~\ref{prob:} by adapting our algorithm for monitoring time-homogeneous (i.e., non time varying) Markov chains.
%Observe that when the impact function is the identity function, i.e., $\impact(\population,\cdot) = \population$ for every $\population\in\features$, then the population remains fixed at the initial population $\population_1$.
%Thus, Prob.~\ref{prob:} reduces to simply estimating the value of the fairness property $\varphi$ for $\population_1$ given the sequence of samples $\set{x_t}_t$ from $\population_1$.
%This problem can be easily solved using an approach that we proposed in an earlier work on monitoring fairness over a given time-homogeneous (i.e., non-time-varying) Markov chain \cite{??}. %, which is summarized below.
%%Afterwards, we show how Prob.~\ref{prob:} can be reduced to the monitoring problem for time-inhomogeneous Markov chains with special structures, and propose a modification
%
%We present an algorithm for solving Prob.~\ref{prob:} when the impact function is not necessarily the identity function.
%The proposed algorithm is adapted from our algorithm for monitoring time-homogeneous Markov chains, where we exploit the fact that Prob.~\ref{prob:} can be reduced to the problem of monitoring fairness on a time-inhomogeneous Markov chain with a special structure.
%
%\subsection{Encoding the Problem in a Markov Chain}
